PolyModel for Hedge Funds' Portfolio Construction Using Machine Learning

The domain of hedge fund investments is undergoing significant transformation, influenced by the rapid expansion of data availability and the advancement of analytical technologies. This study explores the enhancement of hedge fund investment performance through the integration of machine learning techniques, the application of PolyModel feature selection, and the analysis of fund size. We address three critical questions: (1) the effect of machine learning on trading performance, (2) the role of PolyModel feature selection in fund selection and performance, and (3) the comparative reliability of larger versus smaller funds. Our findings offer compelling insights. We observe that while machine learning techniques enhance cumulative returns, they also increase annual volatility, indicating variability in performance. PolyModel feature selection proves to be a robust strategy, with approaches that utilize a comprehensive set of features for fund selection outperforming more selective methodologies. Notably, Long-Term Stability (LTS) effectively manages portfolio volatility while delivering favorable returns. Contrary to popular belief, our results suggest that larger funds do not consistently yield better investment outcomes, challenging the assumption of their inherent reliability. This research highlights the transformative impact of data-driven approaches in the hedge fund investment arena and provides valuable implications for investors and asset managers. By leveraging machine learning and PolyModel feature selection, investors can enhance portfolio optimization and reassess the dependability of larger funds, leading to more informed investment strategies.

==> Link.tex <==
https://www.ssrn.com/index.cfm/en/janda/announcement/?id=14124

==> name.tex <==
class CommunicationException(Exception):
    def __init__(self, message):
        super().__init__(message)

class CommsHandler:
    def __init__(self):
        self.connected_users = []

    def connect(self, user1, user2):
        if user1 == user2:
            raise CommunicationException(f"{user1.name} cannot connect with {user2.name}")
        if self.connected_users:
            raise CommunicationException("Connection in use. Please try later")
        self.connected_users = [user1, user2]
        return f"Connection established between {user1.name} and {user2.name}"

    def hangup(self, user1, user2):
        if user1 == user2:
            raise CommunicationException(f"{user1.name} cannot hangup with {user2.name}")
        if user1 not in self.connected_users or user2 not in self.connected_users:
            raise CommunicationException(f"{user1.name} and {user2.name} not found in the communication channel")
        self.connected_users = []
        return f"{user1.name} and {user2.name} are disconnected"

    def clear_all(self):
        self.connected_users = []
